The Last Eight-Billion Years of Intergalactic CIV Evolution

We surveyed the HST UV spectra of 49 low-redshift quasars for z < 1 CIV candidates, relying solely on the characteristic wavelength separation of the doublet. After consideration of the defining traits of CIV doublets (e.g., consistent line profiles, other associated transitions, etc.), we defined a sample of 38 definite (group G = 1) and five likely (G = 2) doublets with rest equivalent widths W_r for both lines detected at >= 3 sigma. We conducted Monte-Carlo completeness tests to measure the unblocked redshift (dz) and co-moving pathlength (dX) over which we were sensitive to CIV doublets of a range of equivalent widths and column densities. The absorber line density of (G = 1+2) doublets is dN/dX = 4.1+0.7/-0.6 for log N(C^+3) >= 13.2, and dN/dX has not evolved significantly since z = 5. The best-fit power-law to the G = 1 frequency distribution of column densities f(N(C^+3)) = k(N(C^+3)/N_0)^alpha_N has coefficient k = (0.67+0.18/-0.16) x 10^-14 cm^2 and exponent alpha_N = -1.50+0.17/-0.19, where N_0 = 10^14 cm^-2. Using the power-law model of f(N(C^+3)), we measured the C^+3 mass density relative to the critical density: Omega(C^+3) = (6.20+1.82/-1.52) x 10^-8 for 13 <= log N(C^+3) <= 15. This value is a 2.8+/-0.7 increase in Omega(C^+3) compared to the error-weighted mean from several 1 < z < 5 surveys for CIV absorbers. A simple linear regression to Omega(C^+3) over the age of the Universe indicates that Omega(C^+3) has slowly but steadily increased from z = 5 --> 0, with dOmega(C^+3)/dt_age = (0.42+/-0.2) x 10^-8 Gyr^-1.

==> tab1.tex <==
 
 
\begin{deluxetable}{llllllr@{\ }lllllp{1.8cm}p{2.5cm}}
\rotate
\tablecolumns{14}
\tablewidth{0pc}
\tablecaption{OBSERVATION SUMMARY \label{tab.obssumm}}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} & \colhead{(5)} & 
\colhead{(6)} & \multicolumn{2}{c}{(7)} & \colhead{(8)} & \colhead{(9)} & \colhead{(10)} & 
\colhead{(11)} & \colhead{(12)} & \colhead{(13)} \\
\colhead{Target} & \colhead{RA} & \colhead{Dec} & 
\colhead{$\zem$} & \colhead{Instr.} & \colhead{Grating} & 
\multicolumn{2}{c}{$R$ (FWHM)} & 
\colhead{S/N} & \colhead{$\lambda_{\rm min}$} & \colhead{$\lambda_{\rm max}$} & 
\colhead{$t_{exp}$} & \colhead{PID} & \colhead{Notes} \\
 & \colhead{(J2000)} & \colhead{(J2000)} & & & & 
\multicolumn{2}{c}{\hspace{\stretch{1}}(\!\kms)} & 
\colhead{(pix$^{-1}$)} & \colhead{(\AA)} & \colhead{(\AA)} & 
\colhead{(ks)}  & & 
}
\startdata
                   MRK335 &     00:06:19 &    +20:12:10 & 0.0258 & STIS &  E140M &   45800 & $(   7)$ &    7 & 1141 & 1710 &    17 & 9802 &  \\
                     &              &              &        & GHRS &  G160M &   20000 & $(  15)$ &   34 & 1222 & 1258 &    15 & 3584 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  10$ &  904 & 1188 &    99 & P101 &  \\
               Q0026+1259 &     00:29:13 &    +13:16:04 & 0.1450 & GHRS &  G270M &   20000 & $(  15)$ &    5 & 2785 & 2831 &     5 & 3755 & Exclude (coverage) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   2$ &  904 & 1188 &    20 & Q206 &  \\
                  TONS180 &     00:57:20 &   --22:22:56 & 0.0620 & STIS &  G140M &   12700 & $(  24)$ &   25 & 1244 & 1298 &     3 & 7345 & Exclude (coverage) \\
                     &              &              &        &      & G230MB &    9450 & $(  32)$ &    9 & 2758 & 2912 &     1 & 9128 & Exclude (coverage) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   5$ &  904 & 1188 &    25 & D028; P101 & \\
               PG0117+213 &     01:20:17 &    +21:33:46 & 1.4930 & STIS &  E230M &   30000 & $(  10)$ &    8 & 2278 & 3072 &    42 & 8673 &  \\
                  TONS210 &     01:21:51 &   --28:20:57 & 0.1160 & STIS &  E140M &   45800 & $(   7)$ &    6 & 1141 & 1710 &    22 & 9415 &  \\
                     &              &              &        &      &  E230M &   30000 & $(  10)$ &    4 & 1988 & 2782 &     5 & 9415 &  \\
                     &              &              &        &      & G230MB &    9450 & $(  32)$ &    0 & 2759 & 2913 &     2 & 9128 & Exclude ($R$) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   8$ &  904 & 1188 &    53 & P107 & \\
             HE0226--4410 &     02:28:15 &   --40:57:15 & 0.4950 & STIS &  E140M &   45800 & $(   7)$ &    7 & 1141 & 1709 &    44 & 9184 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   7$ &  904 & 1188 &   209 & D027; P101; P207 &  \\
              PKS0232--04 &     02:35:07 &   --04:02:06 & 1.4398 & STIS &  E230M &   30000 & $(  10)$ &    5 & 2278 & 3072 &    42 & 8673 &  \\
               B0312--770 &     03:11:55 &   --76:51:50 & 0.2230 & STIS &  E140M &   45800 & $(   7)$ &    6 & 1141 & 1710 &    38 & 8651 &  \\
                     &              &              &        &      &  E230M &   30000 & $(  10)$ &    2 & 2131 & 2942 &     6 & 8651 &  \\
             PKS0405--123 &     04:07:48 &   --12:11:36 & 0.5726 & STIS &  E140M &   45800 & $(   7)$ &    7 & 1140 & 1709 &    27 & 7576 &  \\
%                     &              &              &        &      &  G230M &   11200 & $(  27)$ &   12 & 1970 & 2058 &     5 & 7290 & Exclude ($R$) \\
                     &              &              &        &      &  G230M &   11600 & $(  26)$ &   13 & 1970 & 2220 &    13 & 7290 &  \\
%                    &              &              &        &      &  G230M &   11600 & $(  26)$ &   12 & 2050 & 2138 &     4 & 7290 & Exclude ($R$) \\
%                    &              &              &        &      &  G230M &   12100 & $(  25)$ &   13 & 2132 & 2220 &     3 & 7290 & Exclude ($R$) \\
                     &              &              &        & GHRS &  G160M &   20000 & $(  15)$ &    3 & 1538 & 1573 &    15 & 6712 & Exclude (overlap) \\
                     &              &              &        &      &  G200M &   20000 & $(  15)$ &    3 & 1701 & 1741 &    15 & 6712 &  \\
                     &              &              &        &      &  G200M &   20000 & $(  15)$ &    3 & 1836 & 1876 &     8 & 6712 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   7$ &  904 & 1188 &   142 & B087; D103 &  \\
              PKS0454--22 &     04:56:08 &   --21:59:09 & 0.5337 & STIS &  E230M &   30000 & $(  10)$ &    4 & 1607 & 2366 &    15 & 8672 &  \\
                     &              &              &        &      & G230MB &    9920 & $(  30)$ &   25 & 2899 & 3051 &    22 & 7475 & Exclude ($R$) \\
                     &              &              &        & GHRS &  G160M &   20000 & $(  15)$ &    1 & 1379 & 1415 &    20 & 5506 &  \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &    2 & 1426 & 1462 &    18 & 5506 &  \\
                     &              &              &        &      &  G200M &   20000 & $(  15)$ &    1 & 1745 & 1785 &    18 & 5506 & Exclude (overlap) \\
                     &              &              &        &      &  G200M &   20000 & $(  15)$ &    3 & 1782 & 1822 &    63 & 5961 & Exclude (overlap) \\
             HE0515--4414 &     05:17:07 &   --44:10:55 & 1.7100 & STIS & G230LB &     910 & $( 329)$ &   41 & 1668 & 3073 &     2 & 9187 & Exclude ($R$) \\
                     &              &              &        &      &  E230M &   30000 & $(  10)$ &   10 & 2303 & 3072 &    32 & 8288 &  \\
             PKS0558--504 &     05:59:47 &   --50:26:53 & 0.1370 & STIS & G230MB &    9450 & $(  32)$ &   11 & 2759 & 2912 &     2 & 9128 & Exclude (coverage) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   7$ &  904 & 1188 &    95 & C149; P101 & \\
              HS0624+6907 &     06:30:02 &    +69:05:03 & 0.3700 & STIS &  E140M &   45800 & $(   7)$ &    8 & 1141 & 1710 &    62 & 9184 &  \\
                     &              &              &        &      & G230MB &    9450 & $(  32)$ &   11 & 2759 & 2912 &     2 & 9128 & Exclude ($R$) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   4$ &  904 & 1188 &   126 & P107; S601; U102 & \\
             QJ0640--5031 &     06:40:56 &   --50:31:46 & 0.2040 & STIS &  E140M &   45800 & $(   7)$ &    1 & 1140 & 1729 &    20 & 7762 & Exclude (low S/N) \\
              HS0747+4259 &     07:50:54 &    +42:52:19 & 1.8971 & STIS &  E230M &   30000 & $(  10)$ &    6 & 2135 & 2942 &    54 & 9040 &  \\
              HS0810+2554 &     08:13:31 &    +25:45:02 & 1.5100 & STIS & G230LB &     910 & $( 329)$ &   15 & 1668 & 3073 &     2 & 9187 & Exclude ($R$) \\
                     &              &              &        &      &  E230M &   30000 & $(  10)$ &    3 & 2135 & 2942 &    53 & 9040 &  \\
               PG0953+415 &     09:56:52 &    +41:15:22 & 0.2341 & STIS &  E140M &   45800 & $(   7)$ &    7 & 1141 & 1730 &    24 & 7747 &  \\
                     &              &              &        &      &  G140M &   11700 & $(  26)$ &   16 & 1146 & 1199 &    13 & 8695 &  \\
                     &              &              &        &      &  G230M &    9830 & $(  30)$ &    9 & 1724 & 1813 &    25 & 8695; 9158 &  \\
                     &              &              &        & GHRS &  G160M &   20000 & $(  15)$ &    4 & 1373 & 1409 &    21 & 6261 & Exclude (overlap) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   8$ &  904 & 1188 &    72 & P101 & \\
                  MARK132 &     10:01:29 &    +54:54:37 & 1.7567 & STIS &  E230M &   30000 & $(  10)$ &   10 & 2278 & 3073 &    69 & 9186 &  \\
                    TON28 &     10:04:02 &    +28:55:35 & 0.3297 & STIS &  E140M &   45800 & $(   7)$ &    6 & 1141 & 1709 &    48 & 9184 &  \\
                     &              &              &        &      &  G230M &   10500 & $(  29)$ &    4 & 1840 & 1928 &     5 & 7290 & Exclude ($R$) \\
                     &              &              &        & GHRS &  G160M &   20000 & $(  15)$ &    3 & 1547 & 1581 &    15 & 6712 & Exclude (overlap) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  2$ &  904 & 1188 &    11 & P207 & Exclude (low S/N) \\
               PG1004+130 &     10:07:26 &    +12:48:56 & 0.2400 & GHRS &  G140L &    2000 & $( 150)$ &   13 & 1272 & 1558 &     6 & 5826 & Exclude ($R$) \\
                     &              &              &        &      &  G270M &   20000 & $(  15)$ &    7 & 2778 & 2824 &    10 & 4223 & Exclude (coverage) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   3$ &  904 & 1188 &    85 & A035 &  \\
                    TON34 &     10:19:56 &    +27:44:01 & 1.9280 & STIS &  E230M &   30000 & $(  10)$ &    2 & 2277 & 3071 &    27 & 9186 & Exclude (low S/N) \\
              HE1029--140 &     10:31:54 &   --14:16:51 & 0.0860 & STIS &  G140M &   12700 & $(  24)$ &   21 & 1244 & 1298 &     3 & 7345 & Exclude (coverage) \\
                  3C249.1 &     11:04:13 &    +76:58:58 & 0.3115 & STIS &  E140M &   45800 & $(   7)$ &    8 & 1141 & 1710 &    69 & 9184 &  \\
                     &              &              &        &      & G230MB &    9450 & $(  32)$ &    4 & 2759 & 2912 &     2 & 9128 & Exclude ($R$) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   3$ &  904 & 1189 &   156 & P107; S601; U102 & \\
            HE1104--1805A &     11:06:33 &   --18:21:25 & 2.3190 & STIS &  E230M &   30000 & $(  10)$ &    1 & 2278 & 3073 &   112 & 8471 & Exclude (low S/N) \\
                  NGC3516 &     11:06:47 &    +72:34:07 & 0.0088 & STIS &  E140M &   45800 & $(   7)$ &    2 & 1141 & 1730 &     5 & 8029 &  \\
                     &              &              &        &      &  E230M &   30000 & $(  10)$ &    4 & 2275 & 3120 &     2 & 8029 &  \\
                     &              &              &        & GHRS &  G160M &   20000 & $(  15)$ &   11 & 1528 & 1597 &    29 & 5724; 5728 &  \\
               PG1116+215 &     11:19:08 &    +21:19:18 & 0.1765 & STIS &  E140M &   45800 & $(   7)$ &   14 & 1140 & 1710 &    40 & 8097; 8165 &  \\
%                     &              &              &        &      &  G140M &   12200 & $(  25)$ &   19 & 1195 & 1248 &     4 & 7345 & Exclude ($R$) \\
                     &              &              &        &      &  G140M &   12450 & $(  24)$ &   23 & 1195 & 1298 &     8 & 7345 & Exclude ($R$) \\
%                     &              &              &        &      &  G140M &   12700 & $(  24)$ &   18 & 1245 & 1298 &     4 & 7345 & Exclude ($R$) \\
                     &              &              &        &      &  E230M &   30000 & $(  10)$ &    8 & 2007 & 2819 &     6 & 8097 &  \\
                     &              &              &        & GHRS &  G140L &    2000 & $( 150)$ &   31 & 1218 & 1504 &    13 & 6499 & Exclude ($R$) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   9$ &  904 & 1188 &    74 & P101 & \\
             HE1122--1648 &     11:24:42 &   --17:05:17 & 2.4000 & STIS &  E230M &   30000 & $(  10)$ &    2 & 2278 & 3072 &    12 & 9885 & Exclude (low S/N) \\
             PKS1127--145 &     11:30:07 &   --14:49:27 & 1.1840 & STIS &  E230M &   30000 & $(  10)$ &    2 & 2278 & 3072 &    52 & 9173 &  \\
                  NGC3783 &     11:39:01 &   --37:44:19 & 0.0097 & STIS &  E230M &   30000 & $(  10)$ &    8 & 2274 & 3119 &     2 & 8029 &  \\
                     &              &              &        & GHRS &  G160M &   20000 & $(  15)$ &   16 & 1232 & 1268 &     8 & 3463 &  \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &    8 & 1527 & 1597 &    27 & 1160; 3936; 5724 &  \\
                     &              &              &        &      &  G270M &   20000 & $(  15)$ &   13 & 2333 & 2381 &    10 & 6500 &  \\
                  NGC4051 &     12:03:09 &    +44:31:52 & 0.0023 & STIS &  E140M &   45800 & $(   7)$ &    3 & 1141 & 1710 &    10 & 8321 &  \\
               PG1206+459 &     12:08:58 &    +45:40:35 & 1.1550 & STIS &  E230M &   30000 & $(  10)$ &    6 & 2277 & 3071 &    17 & 8672 &  \\
                  NGC4151 &     12:10:32 &    +39:24:20 & 0.0033 & STIS &  E140M &   45800 & $(   7)$ &   17 & 1140 & 1710 &    29 & 8019; 8473; 8608; 9272 &  \\
                     &              &              &        &      & G230LB &     910 & $( 329)$ &  141 & 1675 & 3073 &     7 & 7569; 8136 & Exclude ($R$) \\
                     &              &              &        &      &  E230M &   30000 & $(  10)$ &   22 & 2277 & 3072 &     8 & 8019; 8608; 9272 &  \\
                     &              &              &        & GHRS &  G160M &   20000 & $(  15)$ &   25 & 1502 & 1537 &     7 & 2498 & Exclude (overlap) \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &   58 & 1530 & 1565 &    34 & 1141; 4880; 5169 & Exclude (overlap) \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &   21 & 1582 & 1616 &     7 & 2498 & Exclude (overlap) \\
                     &              &              &        &      &  G270M &   20000 & $(  15)$ &   35 & 2772 & 2818 &     4 & 4880; 5169 & Exclude (overlap) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  12$ &  904 & 1188 &    90 & C092; P111; P211 & \\
               PG1211+143 &     12:14:17 &    +14:03:12 & 0.0809 & STIS &  E140M &   45800 & $(   7)$ &   18 & 1141 & 1710 &    67 & 8571 &  \\
                     &              &              &        &      &  G140M &   12450 & $(  24)$ &   21 & 1195 & 1298 &    11 & 7345 & Exclude ($R$) \\
%                     &              &              &        &      &  G140M &   12200 & $(  25)$ &   18 & 1195 & 1248 &     6 & 7345 & Exclude ($R$) \\
%                     &              &              &        &      &  G140M &   12700 & $(  24)$ &   22 & 1245 & 1298 &     5 & 7345 & Exclude ($R$) \\
                     &              &              &        & GHRS &  G140L &    2000 & $( 150)$ &   25 & 1200 & 1486 &     4 & 5947 & Exclude ($R$) \\
                     &              &              &        &      &  G140L &    2000 & $( 150)$ &    1 & 1273 & 1559 &     4 & 5947 & Exclude ($R$) \\
                     &              &              &        &      &  G270M &   20000 & $(  15)$ &    4 & 2788 & 2833 &     1 & 2553 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   8$ &  904 & 1188 &    52 & P107 &  \\
               PG1216+069 &     12:19:21 &    +06:38:38 & 0.3313 & STIS &  E140M &   45800 & $(   7)$ &    6 & 1141 & 1709 &    70 & 9184 &  \\
                     &              &              &        & GHRS &  G140L &    2000 & $( 150)$ &   15 & 1196 & 1482 &     4 & 5947 & Exclude ($R$) \\
                     &              &              &        &      &  G140L &    2000 & $( 150)$ &    4 & 1273 & 1559 &     4 & 5947 & Exclude ($R$) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   2$ &  904 & 1188 &    12 & P107 & \\
                   MRK205 &     12:21:44 &    +75:18:38 & 0.0708 & STIS &  E140M &   45800 & $(   7)$ &    9 & 1141 & 1710 &    78 & 8625 &  \\
                     &              &              &        & GHRS &  G160M &   20000 & $(  15)$ &    4 & 1535 & 1570 &    12 & 2553 & Exclude (overlap) \\
                     &              &              &        &      &  G270M &   20000 & $(  15)$ &    6 & 2784 & 2830 &     3 & 2553 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   7$ &  904 & 1188 &   223 & D054; Q106; S601; U103 &  \\
                  NGC4395 &     12:25:48 &    +33:32:51 & 0.0011 & STIS &  E140M &   45800 & $(   7)$ &    0 & 1141 & 1710 &     8 & 9362 & Exclude (low S/N) \\
                     &              &              &        &      &  E230M &   30000 & $(  10)$ &    1 & 2275 & 3119 &     2 & 9362 & Exclude (low S/N) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  2$ &  904 & 1188 &    37 & C086 & Exclude (low S/N) \\
                    3C273 &     12:29:06 &    +02:03:08 & 0.1583 & STIS &  E140M &   45800 & $(   7)$ &   21 & 1140 & 1709 &    19 & 8017 &  \\
                     &              &              &        & GHRS &  G140L &    2000 & $( 150)$ &   32 & 1174 & 1460 &     1 & 1140 & Exclude ($R$) \\
                     &              &              &        &      &  ECH-A &  100000 & $(   3)$ &    7 & 1250 & 1256 &    20 & 5719 &  \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &   24 & 1522 & 1557 &     6 & 1140; 4883 & Exclude (overlap) \\
                     &              &              &        &      &  G200M &   20000 & $(  15)$ &    7 & 1773 & 1813 &     1 & 1140 &  \\
                     &              &              &        &      &  G270M &   20000 & $(  15)$ &   14 & 2776 & 2822 &     1 & 1140 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  15$ &  904 & 1188 &    42 & P101 &  \\
       QSO--123050+011522 &     12:30:50 &    +01:15:21 & 0.1170 & STIS &  E140M &   45800 & $(   7)$ &    8 & 1141 & 1710 &    27 & 7737 &  \\
                     &              &              &        & GHRS &  G140L &    2000 & $( 150)$ &   30 & 1165 & 1460 &    10 & 6410 & Exclude ($R$) \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &    4 & 1217 & 1253 &    12 & 6410 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  2$ &  904 & 1188 &     1 & P101 & Exclude (low S/N) \\
              Q1230+0947 &     12:33:28 &    +09:31:04 & 0.4200 & GHRS &  G140L &    2000 & $( 150)$ &   13 & 1195 & 1481 &     4 & 5947 & Exclude (coverage) \\
                    &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  1$ &  904 & 1188 &    13 & P207 & Exclude (low S/N) \\
                  NGC4593 &     12:39:39 &   --05:20:39 & 0.0090 & STIS &  E140M &   45800 & $(   7)$ &    4 & 1141 & 1709 &    11 & 8481 &  \\
               PG1241+176 &     12:44:10 &    +17:21:04 & 1.2830 & STIS &  G230L &     740 & $( 405)$ &   28 & 1571 & 3155 &     1 & 8681 & Exclude ($R$) \\
                     &              &              &        &      &  E230M &   30000 & $(  10)$ &    6 & 2277 & 3071 &    19 & 8672 &  \\
               PG1248+401 &     12:50:48 &    +39:51:39 & 1.0320 & STIS &  E230M &   30000 & $(  10)$ &    6 & 2277 & 3071 &    25 & 8672 &  \\
               PG1259+593 &     13:01:12 &    +59:02:06 & 0.4778 & STIS &  E140M &   45800 & $(   7)$ &    9 & 1141 & 1710 &    96 & 8695 &  \\
                     &              &              &        &      &  G140M &   12200 & $(  25)$ &    6 & 1195 & 1249 &     2 & 7295 & Exclude ($R$) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  13$ &  904 & 1188 &   635 & P108; U103 & \\
             PKS1302--102 &     13:05:32 &   --10:33:20 & 0.2784 & STIS &  E140M &   45800 & $(   7)$ &    8 & 1141 & 1729 &    22 & 8306 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   6$ &  904 & 1188 &   146 & P108 &  \\
               PG1307+085 &     13:09:47 &    +08:19:47 & 0.1550 & STIS & G230MB &    9450 & $(  32)$ &    5 & 2759 & 2912 &     2 & 9128 & Exclude (coverage) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   2$ &  904 & 1188 &    10 & P107 & \\
                   CSO873 &     13:19:56 &    +27:28:08 & 1.0140 & STIS &  E230M &   30000 & $(  10)$ &    6 & 2277 & 3073 &    14 & 8672 &  \\
                Q1331+170 &     13:33:35 &    +16:49:02 & 2.0840 & STIS &  E230M &   30000 & $(  10)$ &    5 & 2277 & 3073 &    68 & 7271; 9172 & Exclude (low S/N) \\
                   MRK279 &     13:53:03 &    +69:18:29 & 0.0304 & STIS &  E140M &   45800 & $(   7)$ &   20 & 1141 & 1710 &    55 & 9275; 9688 &  \\
                     &              &              &        & GHRS &  G160M &   20000 & $(  15)$ &   27 & 1223 & 1258 &    20 & 6593 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  18$ &  904 & 1188 &   275 & C090; D154; F325; P108; S601 &  \\
                  NGC5548 &     14:17:59 &    +25:08:12 & 0.0172 & STIS &  E140M &   45800 & $(   7)$ &    8 & 1140 & 1730 &    72 & 7572; 9279; 9511 &  \\
                     &              &              &        & GHRS &  G160M &   20000 & $(  15)$ &   35 & 1232 & 1268 &     5 & 5889 & Exclude (overlap) \\
                     &              &              &        &      &  G140L &    2000 & $( 150)$ &   17 & 1417 & 1703 &     2 & 6485 & Exclude ($R$) \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &   15 & 1520 & 1590 &    24 & 5889; 6485 & Exclude (overlap) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  3$ &  904 & 1188 &    57 & D155; P101 & Exclude (low S/N) \\
                  MRK1383 &     14:29:06 &    +01:17:05 & 0.0865 & STIS &  E140M &   45800 & $(   7)$ &   10 & 1141 & 1709 &    19 & 9778 &  \\
%                     &              &              &        &      &  G140M &   12200 & $(  25)$ &   22 & 1195 & 1248 &     4 & 7345 & Exclude ($R$) \\
                     &              &              &        &      &  G140M &   12450 & $(  24)$ &   26 & 1195 & 1298 &     8 & 7345 & Exclude ($R$) \\
 %                    &              &              &        &      &  G140M &   12700 & $(  24)$ &   26 & 1245 & 1298 &     4 & 7345 & Exclude ($R$) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  12$ &  904 & 1188 &    64 & P101; P267 & \\
               PG1444+407 &     14:46:45 &    +40:35:06 & 0.2673 & STIS &  E140M &   45800 & $(   7)$ &    6 & 1141 & 1710 &    49 & 9184 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  2$ &  904 & 1188 &    10 & P107 & Exclude (low S/N) \\
                  MARK290 &     15:35:52 &    +57:54:09 & 0.0296 & GHRS &  G160M &   20000 & $(  15)$ &    8 & 1232 & 1268 &     7 & 6590 & Exclude (coverage) \\
                Q1553+113 &     15:55:43 &    +11:11:24 & 0.3600 & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   4$ &  904 & 1189 &    47 & E526 & \\
                   MRK876 &     16:13:57 &    +65:43:09 & 0.1290 & STIS &  E140M &   45800 & $(   7)$ &    6 & 1141 & 1710 &    29 & 9754 &  \\
                     &              &              &        &      &  G140M &   12200 & $(  25)$ &   11 & 1195 & 1249 &     2 & 7295 & Exclude ($R$) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  13$ &  904 & 1188 &   143 & D028; P107; U103 & \\
               PG1630+377 &     16:32:01 &    +37:37:49 & 1.4761 & STIS &  E230M &   30000 & $(  10)$ &    7 & 2278 & 3073 &    34 & 8673 &  \\
                     &              &              &        & GHRS &  G140L &    2000 & $( 150)$ &   22 & 1174 & 1460 &    16 & 5177 & Exclude ($R$) \\
               PG1634+706 &     16:34:28 &    +70:31:32 & 1.3340 & STIS &  E230M &   30000 & $(  10)$ &   13 & 1877 & 2673 &    29 & 7292 &  \\
                     &              &              &        &      &  E230M &   30000 & $(  10)$ &   17 & 2277 & 3071 &    26 & 8312 &  \\
              HS1700+6416 &     17:01:00 &    +64:12:09 & 2.7357 & STIS &  E140M &   45800 & $(   7)$ &    2 & 1140 & 1710 &   102 & 7778 &  \\
                     &              &              &        & GHRS &  G140L &    2000 & $( 150)$ &   15 & 1103 & 1388 &    51 & 5328; 6433 & Exclude ($R$) \\
                    3C351 &     17:04:41 &    +60:44:28 & 0.3719 & STIS &  E140M &   45800 & $(   7)$ &    8 & 1141 & 1710 &    77 & 8015 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   4$ &  904 & 1189 &   143 & P108; Q106 &  \\
               PG1718+481 &     17:19:38 &    +48:04:12 & 1.0840 & STIS &  G140M &   15700 & $(  19)$ &    9 & 1541 & 1594 &    11 & 7292 &  \\
                     &              &              &        &      &  E230M &   30000 & $(  10)$ &    9 & 1843 & 2673 &    14 & 7292 &  \\
                     &              &              &        &      & G230MB &    9450 & $(  32)$ &    5 & 2758 & 2912 &     2 & 9128 & Exclude ($R$) \\
                     &              &              &        & GHRS &  G270M &   20000 & $(  15)$ &    9 & 2050 & 2099 &    17 & 5488 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  1$ &  904 & 1188 &    65 & E010; P210 & Exclude (low S/N) \\
                H1821+643 &     18:21:57 &    +64:20:36 & 0.2970 & STIS &  E140M &   45800 & $(   7)$ &    8 & 1141 & 1710 &    51 & 8165 &  \\
                     &              &              &        &      &  G140M &   15700 & $(  19)$ &   14 & 1541 & 1595 &     3 & 8182 & Exclude ($R$) \\
                     &              &              &        &      &  G230M &    9370 & $(  32)$ &   10 & 1643 & 1731 &    16 & 8165 &  \\
%                     &              &              &        &      &  G230M &    9600 & $(  31)$ & **** & 1643 & 1977 &    48 & 8165; 8182 & Exclude ($R$) \\
                     &              &              &        &      &  G230M &   10400 & $(  29)$ &   22 & 1839 & 1928 &    13 & 8182 &  \\
                     &              &              &        &      &  G230M &   10700 & $(  28)$ &   14 & 1889 & 1977 &    10 & 8165 &  \\
                     &              &              &        & GHRS &  G160M &   20000 & $(  15)$ &   10 & 1232 & 1268 &    18 & 4094; 5299 & Exclude (overlap) \\
                     &              &              &        &      &  G140L &    2000 & $( 150)$ &    4 & 1247 & 1533 &    37 & 6155 & Exclude ($R$) \\
                     &              &              &        &      &  G270M &   20000 & $(  15)$ &    9 & 2776 & 2822 &     3 & 4094 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   9$ &  904 & 1188 &   494 & C095; I811; M103; M114; M717; M727; P101; S202; U104 &  \\
             PKS2005--489 &     20:09:25 &   --48:49:54 & 0.0710 & STIS &  G140M &   12700 & $(  24)$ &   40 & 1244 & 1298 &     5 & 7345 & Exclude (coverage) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   7$ &  904 & 1189 &    49 & C149; P107 & \\
                   MRK509 &     20:44:09 &   --10:43:24 & 0.0344 & STIS &  E140M &   45800 & $(   7)$ &    8 & 1141 & 1710 &     8 & 8877 &  \\
                     &              &              &        &      &  E230M &   30000 & $(  10)$ &   10 & 2274 & 3119 &     3 & 8877 &  \\
                     &              &              &        & GHRS &  G160M &   20000 & $(  15)$ &    4 & 1179 & 1215 &     6 & 6412 & Exclude (overlap) \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &    8 & 1219 & 1255 &    11 & 3463; 6593 & Exclude (overlap) \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &   84 & 1232 & 1268 &    11 & 3463; 6593 &  \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &    5 & 1301 & 1337 &     4 & 6412 & Exclude (overlap) \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &    5 & 1382 & 1418 &     5 & 6412 & Exclude (overlap) \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &    6 & 1521 & 1557 &     8 & 5300 & Exclude (overlap) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  12$ &  904 & 1188 &   114 & P108; X017 & \\
             IR2121--1757 &     21:24:41 &   --17:44:45 & 0.1120 & STIS &  E140M &   45800 & $(   7)$ &    1 & 1140 & 1710 &     5 & 7617 & Exclude (low S/N) \\
                  PHL1811 &     21:55:01 &   --09:22:24 & 0.1900 & STIS &  E140M &   45800 & $(   7)$ &   11 & 1141 & 1710 &    34 & 9418 &  \\
                     &              &              &        &      & G230MB &    9450 & $(  32)$ &   14 & 2758 & 2912 &     1 & 9128 & Exclude ($R$) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   8$ &  980 & 1188 &    72 & P108; P207 & \\
             PKS2155--304 &     21:58:51 &   --30:13:32 & 0.1160 & STIS &  E140M &   45800 & $(   7)$ &   17 & 1140 & 1729 &    28 & 8125 &  \\
                     &              &              &        & GHRS &  G140L &    2000 & $( 150)$ &   47 & 1174 & 1460 &     4 & 1172 & Exclude ($R$) \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &   11 & 1223 & 1258 &     5 & 3965 &  \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &    9 & 1258 & 1293 &     7 & 6593 &  \\
                     &              &              &        &      &  G140L &    2000 & $( 150)$ &   29 & 1436 & 1723 &     4 & 1172 & Exclude ($R$) \\
                     &              &              &        &      &  G160M &   20000 & $(  15)$ &   13 & 1520 & 1555 &     7 & 5889 &  \\
                     &              &              &        &      &  ECH-B &  100000 & $(   3)$ &    9 & 2594 & 2606 &     6 & 3965 &  \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le  17$ &  904 & 1189 &   122 & P108 &  \\
 HDFS--223338--603329-QSO &     22:33:37 &   --60:33:28 & 2.2380 & STIS &  E230M &   30000 & $(  10)$ &    1 & 2303 & 3073 &   151 & 8058; 8073; 8074; 8075 & Exclude (low S/N) \\
                   AKN564 &     22:42:39 &    +29:43:31 & 0.0247 & STIS &  E140M &   45800 & $(   7)$ &    3 & 1141 & 1710 &    10 & 8265 & Exclude (low S/N) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   3$ &  904 & 1188 &    61 & B062 & Exclude (low S/N) \\
                  NGC7469 &     23:03:15 &    +08:52:25 & 0.0163 & STIS &  E140M &   45800 & $(   7)$ &    9 & 1141 & 1710 &    36 & 9095; 9802 &  \\
                     &              &              &        &      & G230MB &    9450 & $(  32)$ &   10 & 2758 & 2912 &     1 & 9128 & Exclude ($R$) \\
                     &              &              &        & {\it FUSE} &   LWRS &   20000 & $(  15)$ & $\le   6$ &  917 & 1188 &    45 & C090; P101 & \\
               PG2302+029 &     23:04:45 &    +03:11:46 & 1.0440 & STIS & G230LB &     910 & $( 329)$ &   61 & 1674 & 3071 &     6 & 7358 & Exclude ($R$) \\
                     &              &              &        &      &  E230M &   30000 & $(  10)$ &    2 & 1988 & 2781 &     2 & 7358 & Exclude (low S/N) \\
\enddata
\tablecomments{
The targets and spectra included in the current survey.
The targets, their coordinates, and their redshifts are listed in Columns 1--4.
The instrument and grating of the archived observations (Columns 5 and 6) are listed with the resolution $R$ (and FWHM in \!\kms), exposure time $t_{exp}$, and the proposal identification number (PID) from the MAST query (Columns 7, 11, and 12).
The signal-to-noise ratio S/N was measured from the normalized spectra (Column 8).
Columns 9 and 10 are the wavelength coverage of each spectrum.
The status of the spectra (\ie whether it was excluded and why) is listed in Column 13.
}
\end{deluxetable}
